Fast Hamiltonicity checking via bases of perfect matchings

For an even integer t \geq 2, the Matchings Connecivity matrix H_t is a matrix that has rows and columns both labeled by all perfect matchings of the complete graph K_t on t vertices; an entry H_t[M_1,M_2] is 1 if M_1\cup M_2 is a Hamiltonian cycle and 0 otherwise. Motivated by the computational study of the Hamiltonicity problem, we present three results on the structure of H_t: We first show that H_t has rank at most 2^{t/2-1} over GF(2) via an appropriate factorization that explicitly provides families of matchings X_t forming bases for H_t. Second, we show how to quickly change representation between such bases. Third, we notice that the sets of matchings X_t induce permutation matrices within H_t. Subsequently, we use the factorization to obtain an 1.888^n n^{O(1)} time Monte Carlo algorithm that solves the Hamiltonicity problem in directed bipartite graphs. Our algorithm as well counts the number of Hamiltonian cycles modulo two in directed bipartite or undirected graphs in the same time bound. Moreover, we use the fast basis change algorithm from the second result to present a Monte Carlo algorithm that given an undirected graph on n vertices along with a path decomposition of width at most pw decides Hamiltonicity in (2+\sqrt{2})^{pw}n^{O(1)} time. Finally, we use the third result to show that for every \epsilon >0 this cannot be improved to (2+\sqrt{2}-\epsilon)^{pw}n^{O(1)} time unless the Strong Exponential Time Hypothesis fails, i.e., a faster algorithm for this problem would imply the breakthrough result of a (2-\epsilon)^n time algorithm for CNF-Sat.

==> packages.tex <==

\usepackage[utf8x]{inputenc}

\usepackage{tikz}
\usepackage{rotating}
\usepackage{xspace}
\usepackage{array}
\usepackage{paralist}
\usepackage{fullpage}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{etex}
\usepackage{graphicx}
\usepackage{paralist}

\usepackage[noend]{algorithmic}
\usepackage[boxed]{algorithm}

\usepackage{color}

\usepackage{fullpage}

==> randomized-conclusions.tex <==
\section{Conclusions}\label{section:conclusions}

We have presented a set of matchings $\basis_n$,
which forms a basis of the \hamiltonianmatrix~$\HC_n$.
In particular we have obtained a factorization
theorem (Theorem~\ref{theorem:hmatrixfactorization})
which shows an explicit way of expressing any perfect
matching as a linear combination of matchings of $\basis_n$.
As a consequence we obtained deterministic algorithms
for computing the parity of the number of Hamiltonian
cycles in undirected graphs and directed bipartite graphs
in $\Oh(\hcconst^n)$, which together with the Isolation
Lemma lead to Monte Carlo algorithms solving the decision versions
of Hamiltonicity within the same running time.
Moreover, using the basis $\basis_n$,
we presented an algorithm which given an undirected graph 
on $n$ vertices along with a path decomposition 
of width at most $\pw$, decides Hamiltonicity in $(2+\sqrt{2})^{\pw}n^{\Oh(1)}$ time.
Somewhat surprisingly we use the same tool, i.e. the basis $\basis_n$,
to show by an involved reduction from CNF-Sat that our bounded pathwidth algorithm
is optimal under the Strong Exponential Time Hypothesis.

Our results lead to several natural open problems.
Can the basis $\basis_n$ be used to obtain a deterministic
$\Oh((2-\epsilon)^n)$ time algorithm for Hamiltonicity?
Can we handle directed graphs without the bipartiteness assumption?
Can we extend our bounded pathwidth algorithm to a bounded treewidth algorithm
with the same complexity?

Finally we would like to note that the row space of the
\hamiltonianmatrix~$\HC_n$ clearly has several different 
bases. We have investigated a particular one, which 
proved to have several interesting properties
and applications, however there might be different
ones which are also worth exploring.

\section*{Acknowledgements}

We would like to thank Marcin Pilipczuk, Micha\l{} Pilipczuk, Johan van Rooij and Jakub Onufry Wojtaszczyk for early discussions on Section~\ref{section:hamcycle:lowerbound}.

==> randomized-introduction.tex <==
\section{Introduction}

The Hamiltonicity problem and its generalization to the traveling salesman problem are widely acknowledged to be two of the most famous NP-complete
problems. Many classical algorithms were invented to tackle these problems (and variants thereof), among them Cristofides' approximation algorithm~\cite{Chr76}, the
Lin-Kernighan heuristic~\cite{linkerheur73}, and a polynomial time approximation scheme for Euclidean TSP~\cite{Arora:1998:PTA:290179.290180}.

A very early and classical result belonging to this list is due to Bellman~\cite{bellman1958combinatorial,Bellman62} and, independently, Held and
Karp~\cite{Held:1961:DPA:800029.808532}; it demonstrates that the traveling salesman problem can be solved in $\Oh(n^22^n)$ time, where $n$ denotes the
number of vertices of the input graph. In order to get this result they introduced dynamic programming over subsets, which became a fundamental design paradigm for obtaining exact exponential time algorithms (see for example \cite{DreyfWagn} and \cite[Chapter 3]{Fominbook}). Considerable effort has been taken to improve these algorithms: More space efficient
algorithms were already given independently by several authors \cite{Bax1993203,KarpDynIncEx,Kohnetal}.

In his influential survey, Woeginger~\cite{DBLP:conf/aussois/Woeginger01} brought renewed attention to a question suggesting itself already from the 60's: Can
either the traveling salesman problem or the Hamiltonicity problem be solved in $(2-\epsilon)^n n^{\Oh(1)}$ for some $\epsilon > 0$? An affirmative answer
was given for the special cases of bounded degree~\cite{eppstein-tsp-cubic,DBLP:journals/mst/BjorklundHKK10,iwama-tsp-cubic,gebauer-tsp-bound} and claw-free
graphs~\cite{DBLP:conf/wg/BroersmaFHP09}. In a breakthrough result, Bj\"orklund~\cite{DBLP:conf/focs/Bjorklund10} partially resolved the open question by giving
an $1.66^n n^{\Oh(1)}$ time Monte Carlo algorithm deciding undirected Hamiltonicity, using as a first step a $2^{n/2} n^{\Oh(1)}$ time algorithm for bipartite graphs.
Unfortunately, it seems hard to derandomize this result or to extend it to the traveling
salesman problem without incurring a pseudo-polynomial dependence on the input weights.
The algorithm of~\cite{DBLP:conf/focs/Bjorklund10} instead of keeping track of all the vertices along the 
so far constructed path (as Bellman, Held and Karp), labels only some vertices and some edges used on the path.
Bj\"orklund's algorithm uses counting modulo two as a tool for canceling unwanted self-crossing walks,
however it relies on the assumption that the Hamiltonian cycles under consideration satisfy
particular counting invariants concerning the number of vertices and edges used.
For this reason the algorithm of~\cite{DBLP:conf/focs/Bjorklund10}, to the best of our knowledge,
can not determine the parity of the number of all Hamiltonian cycles.

%Also, even though his result crucially depends on dynamic
%programming and improves a dynamic programming result, it did not give any further insight into the optimal substructure. \todo{stefan: can we elaborate? it sounds a bit harsh}

Recall that the algorithm of~\cite{bellman1958combinatorial,Bellman62,Held:1961:DPA:800029.808532} uses dynamic programming based on the observation
that if we have constructed a path from $v_a$ to $v_b$, then the only additional information needed is the set of vertices used along the way.
Hence the essential information required to store for all subpaths is their endpoints and the set of visited vertices, leading to $\Oh(n2^n)$ table entries. Recall that
for designing a fast dynamic programming algorithm, it is essential that one chooses the right strategy of decomposing a candidate solution. For example, if $G$
has a small balanced separator\footnote{A vertex set $X$ such after removing $X$, all connected components have size at most $|V|/2$.} of size $0.1|V|$ it seems
impossible to modify the above algorithm in order to exploit this fact.

In this work we study the following way to decompose a Hamiltonian cycle $H$: Consider an arbitrary ordering $e_1,\ldots,e_m$ of the edges $E$ and decompose
$H$ for every $i$ into $H_1=\{e_1,\ldots,e_i\} \cap H$ and $H_2=\{e_{i+1},\ldots,e_n\} \cap H$. This suggests another dynamic programming strategy
alternative to~\cite{bellman1958combinatorial,Bellman62,Held:1961:DPA:800029.808532} that was much less well-studied, mainly because it seemed a priori that the
essential information needed to store for a set of partial solutions $H_1$ is $2^{\theta(n \lg n)}$: The degrees (zero, one, or two) of each vertex with respect to~$H_1$ and the pairing in which vertices of degree one are connected by~$H_1$. The informed reader will notice that this way of
decomposing solutions is inherent to dynamic programming algorithms that operate on \emph{tree decompositions} or \emph{path decompositions}.


The notions of \emph{pathwidth}/\emph{treewidth} proved to be an excellent tool for dealing with many NP-hard problems on graphs. In the 1970s and 1980s,
several groups of researchers discovered the concept independently. In their fundamental work on graph minors, Robertson and Seymour \cite{Robertson84}
introduced the notions \emph{path/treewidth} and \emph{path/tree decomposition}, and these became the dominant terminology. A graph having small path/treewidth
means informally that it can be decomposed efficiently in a path/tree-like manner. Many problems can be solved using dynamic programming by decomposing a
solution according to the given path/tree decomposition. We refer to~\cite{bodlaendersurvey} for more information on these notions. 

In early work, such as the influential result of Courcelle~\cite{DBLP:journals/iandc/Courcelle90}, algorithms with running times of the type $f(\pw)n$ were given\footnote{Assuming an input
graph $G$ on $n$ vertices along with a path decomposition of $G$ width $\pw$ is given.}. Later it was noticed that for many such algorithms the function $f(\pw)$
can be substantially improved, greatly improving the tractability as well. For example for many problems whose solutions can be verified by separately
considering its intersection with all neighborhoods of the vertices of the input graph (see~\cite{DBLP:conf/podc/GoosS11}), we can obtain
$2^{\Oh(\pw)}n^{\Oh(1)}$ by employing dynamic programming. For example the Independent Set, or equivalently, Vertex Cover, problem can be solved in $2^{\pw}n$
time~\cite{kleinberg-tardos, Niedermeier02invitationto}. From the work of \cite{ImpagliazzoPZ01}
and standard Karp-reduction it follows that this dependence cannot be improved to sub-exponential algorithms unless the Exponential Time Hypothesis fails, i.e., unless
CNF-SAT has a subexponential algorithm. In \cite{treewidth-lower} it was shown that under a stronger assumption (the so-called Strong Exponential
Time Hypothesis (SETH)), the current algorithms are optimal even with respect to polynomial jumps, that is, problems with current best
running time $f(\tw)n^{\Oh(1)}$ cannot be solved in $f(\tw)^{1-\epsilon}n^{\Oh(1)}$ for positive $\epsilon$ where $f(\tw)$ is $2^{\tw}$, $3^{\tw}$ for respectively Independent Set and
Dominating Set.

For the Traveling Salesman problem, or even the Hamiltonian cycle problem, the situation is different since they are not local problems (see for example \cite[Section
5]{DBLP:conf/podc/GoosS11}). In~\cite{Catalan}, the notion of a Catalan structure was introduced to give an algorithm that solves the $k$-path problems on
$H$-minor free graphs in $2^{\Oh(\tw)}$ time. To obtain this, their result works for `pairing-encodable' problems (i.e. problems where the connectivity properties
can be encoded by a matching/pairing) since it bounds the number of ways paths can intersect with a part of the tree decomposition. However, in~\cite{DBLP:conf/focs/CyganNPPRW11} it was shown that along with many other connectivity problems, Hamiltonian cycle can
be solved by a Monte Carlo algorithm in $4^{\Oh(\tw)}n^{\Oh(1)}$ time. For many of these algorithms with running time $f(\tw)n^{\Oh(1)}$, it was shown that
an algorithm running in time $f(\tw)^{1-\epsilon}n^{\Oh(1)}$ would violate SETH. Nevertheless, the exact complexity of the Hamiltonian cycle problem remained elusive.

Recently, a superset of the current authors, found a connection of the optimal substructure of a dynamic programming algorithm
with the rank of a certain matrix~\cite{deterministic}: Consider a matrix $\HC$ with rows and columns indexed by partial solutions, with a $1$ if and only if
the two partial solutions combined give a valid solution, then if we have more than $\rk(\HC)$ partial solutions, one will be redundant in the sense that we can
safely forget it. This leads to deterministic~$2^{\Oh(\tw)}n^{\Oh(1)}$ time algorithms for many connectivity problems, in a sense derandomizing the work of Cygan et al.~\cite{DBLP:conf/focs/CyganNPPRW11}, but the used techniques do not match their runtimes, e.g., the $4^{\tw}n^{\Oh(1)}$ time for Hamiltonian cycle.
 
\subsection*{Our contribution}
Inspired by the mentioned result from~\cite{deterministic}, we study a matrix that we call the \emph{\hamiltonianmatrix}. 
We present a family of perfect matchings $\basis_t$,
which we show to be a basis of the \hamiltonianmatrix, therefore we establish its rank.
All further results of the paper use the basis $\basis_t$ and its properties as its key tool,
which we now elaborate on.

\paragraph{Determining rank of the \hamiltonianmatrix.} For an even integer $t \geq 2$, the \hamiltonianmatrix~$\HC_t$ is a matrix that has rows and columns both
labeled by all perfect matchings of the complete graph~$K_t$ on~$t$ vertices; an entry~$\HC_t[M_1,M_2]$ is~$1$ if~$M_1\cup M_2$ is a Hamiltonian cycle and~$0$
otherwise. The centerpiece of our work is that~$\HC_t$ has rank exactly $2^{t/2-1}$ over GF(2). To establish this result, we define an explicit family~$\basis_t$ of~$2^{t/2-1}$ perfect matchings on~$K_t$ and show that its columns (or rows) form a basis of~$\HC_t$ over GF(2): First, essentially by design, each matching~$M\in\basis_t$ has a unique partner~$M'\in\basis_t$ such that their union is a Hamiltonian cycle. Thus, the rows and columns labeled by~$\basis_t$ induce a permutation matrix, which implies the required rank lower bound. Second, we give an explicit factorization of $\HC_t$ into a product of two rectangular matrices with inner dimensions indexed by~$\basis_t$ in Theorem~\ref{theorem:hmatrixfactorization}. This proves that~$\basis_t$ is indeed a basis, provides an explicit formula for linear combinations, and completes the claimed rank bound (see Section~\ref{section:matchingbasis}).

In~\cite{DBLP:journals/combinatorica/RazS95} a matrix $\HC'_t$ is studied that is obtained by restricting $\HC_t$ to all perfect matchings of the complete \emph{bipartite} graph
with independent sets of size $t/2$. There it is shown that when taken over the reals, the rank of $\HC'_t$ is exactly $\binom{t-1}{t/2-1}$ using
group representation theory. Using this the authors disprove the original\footnote{A weakened version is still a standing open problem in communication
complexity~\cite[Section 13.2]{arora09}.} `log-rank conjecture' in communication complexity since they also showed that the non-deterministic communication
complexity of determining whether two such matchings give a Hamiltonian cycle is $\Omega(n \log \log n )$. In~\cite[Lemma 3.13]{deterministic} a factorization
of a matrix that contains~$\HC_t$ as submatrix into two matrices with inner dimension $2^{t-1}$ was given.

% The centerpiece of our results is a basis for the \hamiltonianmatrix~$\HC_t$ (for each even integer~$t$), which implies that its rank is exactly~$2^{t/2-1}$ over GF(2). The lower follows since the basis matchings themselves induce a submatrix of~$\HC_t$ that is a permutation matrix (and hence of full rank). More strongly, we are able to factorize the matrix as a product of two submatrices that are obtained by restricting either rows or columns to the perfect matchings of our basis. Thus we have an efficient way of computing the linear combination of basis matchings for any other perfect matching (on~$t$ vertices).

% \todo{can we state the theorem without too much information overload?} J:Would not like to define the basis here and besides that we give all info already...

\paragraph{Exact algorithms for Hamiltonicity.}

By exploiting the peculiar form of the basis $\basis_n$ we show
that the number of distinct subsets of all the matchings of $\basis_n$ is $\Oh(\hcconst^n)$.
Together with Theorem~\ref{theorem:hmatrixfactorization} this allows us to show deterministic algorithms computing the parity of the
number of Hamiltonian cycles in undirected graphs and directed bipartite graphs (section~\ref{ssec:mainlemmaproofs}) in $\hcconst^n n^{\Oh(1)}$ time.
By combining those results with the Isolation Lemma
we obtain Monte Carlo algorithms solving the decision version of Hamiltonicity
in both undirected and directed bipartite graphs within the same running time.

Even though our algorithm for undirected graphs is slower than the algorithm of Bj\"orklund~\cite{DBLP:conf/focs/Bjorklund10}, we believe it is of interest
as it uses very much different tools and allows solving the problem also
in directed bipartite graphs. We would like to recall
that solving the Hamiltonicity problem on undirected bipartite graphs
in $\Oh((2-\epsilon)^n)$ time was the first step of Bj\"orklund
on the way to the algorithm for general undirected graphs. 
For this reason we believe that studying directed bipartite graphs
is justified.

\paragraph{Algorithm for bounded pathwidth.} Using the set of perfect matchings~$\basis_t$ we obtain a faster algorithm for solving the Hamiltonian cycle problem
via a non-trivial pathwidth dynamic programming routine. Regarding the algorithm, already from the rank bound it can be argued that only~$(2+\sqrt{2})^{\pw}$
space is needed to solve Hamiltonian cycle on a graph with given path decomposition of width~$\pw$. The key idea is to replace memoization of all partial
solutions by storing only fingerprints of groups of solutions that encode how many partial solutions are consistent with a given basis matching. In fact, these numbers are stored only modulo two which requires only one bit per basis matching. To achieve also \emph{time}~$(2+\sqrt{2})^{\pw}n^{\Oh(1)}$ we show in Lemma~\ref{lemma:basischange} how to efficiently convert these fingerprints
from one basis to another, which permits us to perform the needed dynamic programming table computations (in particular insertion of edges into partial
solutions); this crucially depends on the structure of~$\basis_t$. Notably, Lemma~\ref{lemma:basischange} gives a second proof of the rank upper bound for $\HC_t$, but it does so in a more implicit way; in particular it does not provide an explicit factorization (see Section~\ref{section:hcalgorithm}).

Let us point out the main differences to the related algorithmic results obtained by Bodlaender et al.~\cite{deterministic}: The present faster algorithm for Hamiltonicity parameterized by pathwidth required a new dynamic programming strategy, unlike the results of~\cite{deterministic} that speed up existing formulations. Furthermore, we require randomization (for the Isolation Lemma~\cite{isolation}) to guarantee a unique solution, in order for the fingerprinting approach to work. Finally, achieving time~$(2+\sqrt{2})^{\pw}n^{\Oh(1)}$ depends crucially on the structure of our basis matchings~$\basis_t$ (to allow for Lemma~\ref{lemma:basischange}) and does not appear to follow directly from the rank. (Similarly, the subsequent lower bound requires the existence of a sufficiently large permutation/identity matrix in~$\HC_t$ and does not follow directly from the rank lower bound.)

\paragraph{Matching lower bound assuming SETH.} We show that if the running time of our algorithm can be significantly improved, then satisfiability of CNF-Sat formula's
of $m$ clauses and $n$ vertices can be determined in $(2-\epsilon)^{n}m^{\Oh(1)}$ time. The latter would contradict the \emph{Strong Exponential Time Hypothesis
(SETH)} introduced in~\cite{ImpagliazzoPZ01}. Although there is not consensus about it's truth, a number of results have been given assuming
SETH~\cite{patrascu10sat-lbs,DBLP:conf/coco/CyganDLMNOPSW12,treewidth-lower,DBLP:conf/focs/CyganNPPRW11}. As with previous results, this result should be interpreted that there is a boundary to significantly improving our algorithm, namely finding the so far elusive~$(2-\epsilon)^{n}m^{\Oh(1)}$ algorithm for CNF-Sat.

For the tight runtime lower bound we use our basis as a part of a gadget in a reduction from CNF-Sat. Although the basic setup is similar to previous lower bounds~\cite{treewidth-lower,DBLP:conf/focs/CyganNPPRW11} our reduction is different in the sense that we require a very generic gadget (the induced subgraph gadget, discussed in Subsection~\ref{subsection:lowerbound:gadgets}). Using this, we can exploit  the crucial property that the submatrix of the
\hamiltonianmatrix that is induced by the columns and rows of~$\basis_t$ is a permutation matrix, i.e., each basis matching has a unique partner in~$\basis_t$
such that their union is a Hamiltonian cycle. Then, in a similar but technically challenging vein to the reductions of~\cite{treewidth-lower,DBLP:conf/focs/CyganNPPRW11}, choices can be
transferred through a series of gadgets (see Section~\ref{section:hamcycle:lowerbound}).

\paragraph{Further algorithmic conclusions.}

As a corollary of our bounded pathwidth algorithm in Section~\ref{section:hcalgorithm} (Corollary~\ref{cor:hccub})
we also obtain a $(2+\sqrt{2})^{n/6}n^{\Oh(1)}=1.1583^{n}n^{\Oh(1)}$ time Monte Carlo algorithm for Hamiltonicity in cubic graphs,
which to the best of our knowledge is the fastest known algorithm in this class of graphs.

